Video Fill In the Blank using LR/RL LSTMs with Spatial-Temporal Attentions

Given a video and a description sentence with one missing word (we call it the "source sentence"), Video-Fill-In-the-Blank (VFIB) problem is to find the missing word automatically. The contextual information of the sentence, as well as visual cues from the video, are important to infer the missing word accurately. Since the source sentence is broken into two fragments: the sentence's left fragment (before the blank) and the sentence's right fragment (after the blank), traditional Recurrent Neural Networks cannot encode this structure accurately because of many possible variations of the missing word in terms of the location and type of the word in the source sentence. For example, a missing word can be the first word or be in the middle of the sentence and it can be a verb or an adjective. In this paper, we propose a framework to tackle the textual encoding: Two separate LSTMs (the LR and RL LSTMs) are employed to encode the left and right sentence fragments and a novel structure is introduced to combine each fragment with an "external memory" corresponding the opposite fragments. For the visual encoding, end-to-end spatial and temporal attention models are employed to select discriminative visual representations to find the missing word. In the experiments, we demonstrate the superior performance of the proposed method on challenging VFIB problem. Furthermore, we introduce an extended and more generalized version of VFIB, which is not limited to a single blank. Our experiments indicate the generalization capability of our method in dealing with such more realistic scenarios.

==> ImplementationDetails.tex <==

We used Caffe~\cite{jia2014caffe} to extract all features mentioned above.
\vspace{-3mm}
\subsubsection{Implementation Framework}
This network has been developed under Keras framework~\cite{Charles2013} with Theano ~\cite{2016arXiv160502688short} backend. Categorical Cross-Entropy has been used as the objective function and the network is trained end-to-end by AdaGrad~\cite{duchi2011adaptive} optimizer. All the experiments had been run on an NVIDIA TITAN-X GPU. The batch size had been set to $32$ and training data had been shuffled for each epoch. We used the loss on the validation set after each epoch and use it as an early-stopping criterion. Also, all the parameters of the model had been initialized randomly by Glorot-Unifrom ~\cite{glorot2010understanding} method.


==> bak.tex <==
\subsection{Attribute Attention} \label{AttrSel}

Up to now, the spatial and temporal attentions have discussed. Now we discuss the possibility of benefiting from mid-level knowledge from the video. Mid-level knowledge can be visual attributes, textual data, or any other form of information that we can directly extract from the video. In this work, we have used attributes for question answering task. Attributes can be directly or indirectly informative about the missing word of a sentence. Sometimes an attribute can be as same as the desired blank, but in many cases, it can be a clue to find the correct one; However, it is imperative how to select the useful attributes regarding a given question. For example, a movie scene about a party is more likely to have a correlation with attributes like "Happy face" rather than "Crying face", however, it may correlate with many other attributes as well. The point is to select the attributes which are related based on the question and other visual features which we extracted in previous sections.
\begin{figure} 
\begin{center}
   \includegraphics[width=1 \linewidth]{Figures/Attributes.pdf}

\end{center}
   \caption{Spatial and temporal representations plus encoded  question vector produce coefficients for attribute scores. }
\label{fig:AttrSelFig} 
\end{figure}

Let's denote the list of attributes as $\mat{A} = [a_1,a_2,...a_{|A|}]$ where $|A|$ is the number of attributes and $a_i$ is the confidence score of $i$'th attribute. The main idea is finding one coefficient for each as a relevance factor for that particular attribute. In our approach, we find attributes coefficients respecting our three other sources which are the question, spatial and temporal model. In essence, we are looking for vector $\mat{c} \in \mathbb{R}^{|A|}$:
\begin{equation}
    \mat{c} = \Psi(\mat{u}_{q}, \mat{u}_{Te}, \mat{u}_{Sp})
\end{equation}
Where:
\begin{equation} \label{psi}
    \Psi(\mat{u}, \mat{u}_{Te}, \mat{u}_{Sp}) = ReLU(\mat{W}_c \times \mat{\phi}_c)
\end{equation}
And the vector $\mat{\phi}_c \in \mathbb{R}^{|A| \times d}$, is the summation of the aforementioned clues:
\begin{equation*}
    \mat{\phi}_c =  [\mat{u}_q + \mat{u}_{Te} + \mat{u}_{Sp}]
\end{equation*}
The $ReLU$ activation function give more sparsity more than other activation functions~\cite{glorot2011deep}. It gives more chance to have a zero coefficient for many of the attributes by making the vector $\mat{c}$ more sparse and aids the selection process more effective. Finally, the outcome of the attributes is represented as:
\begin{equation} \label{eq:attrout}
    \mat{u}_{Attr} = \tanh(\mat{W}_{Attr} \times (\mat{c} \odot \mat{A}))
\end{equation}
Where $\mat{W}_{Attr} \in \mathbb{R}^{d \times |A|}$ applied on output of element-wise product of the coefficient vector $\mat{c}$ with attributes detectors scores $\mat{A}$ (See Fig. ~\ref{fig:AttrSelFig}).




==> related.tex <==

%Traditional visual understanding were mostly based on capturing hand-crafted visual features (e.g. SIFT, STIP), to solve tasks like recognizing objects, actions, attributes and etc. Later, researchers became more interested to discovering more knowledge of learning methods and a new variety of problems like object detection and temporal action localization. These tasks introduced many more approaches in machine learning and computer vision and showed that a fine learning mechanism can not only recognize a visual concept, it can also tell where and when it happens.

%By emerging big data-sets like\cite{deng2009imagenet}, Deep Learning algorithms showed a superiority over tradition methods and could exceed the previous state-of-the-art methods. On the other hand, recurrent neural networks and some of its special cases like Long Short Term Memory (LSTM), has shown a wonderful accuracy in modeling repetitive dynamic sequences and specifically the textual information. These advances, lead the researchers to define new problems, specifically problems that encounter both textual and visual patterns. Caption generation became one of the most popular problems recently where generally a deep LSTM is trained to capture the visual representation of an image or video and produce words of a sentence one by one as an output caption. Satisfying caption generation results showed the capability of deep learning models to understand both visual and textual information and it led many researchers to a more interesting problem known as Visual Question Answering (VQA), where the task is to answer a question asked about an image or video. Answering questions needs better understanding of the visual inputs rather than the caption generation since a question can be asked about any details of an image however a good caption can be about a very obvious object or the general information of the scene.

%FIB as explained in -reference to data-set technical report-, can be a good form of question since it is cheaper to build given a list of favor answers. Also, any form of words can be the subject of an FIB question. 

Deep Convolutional Neural Networks (CNNs) ~\cite{krizhevsky2012imagenet,Simonyan2014,szegedy2015going, he2015deep} have gain dramatic success in computer vision, for detection (e.g. object detection ~\cite{deng2009imagenet}) and classification (e.g. action classification  ~\cite{soomro2012ucf101}). And Recurrent Neural Networks (RNN) ~\cite{schuster1997bidirectional,hochreiter1997long, chung2014empirical} has been demonstrated useful in Natural Language Processing (NLP), for translation. Recently, new problems such as Visual Captioning (VC) ~\cite{Xu2015,Venugopalan2014, vinyals2015show}, Visual Question Answer (VQA) have drawn a lot of attention, as these are very challenging problems and are extremely valuable for both computer vision and natural lauguage processing. Both Visual Captioning and Visual Question Answer are related to the Video-Fill-in-the-Blank (VFIB) problem. 

Visual Captioning (VC) needs deep understanding for both visual cues (i.e. image or video) and textual cues. Many approaches for VC has been introduced recently. Some of these algorithms focus on leveraging RNNs which takes visual input and produces words one by one. Another type of approaches, has the benefits to focus on different spatial locations and leverage attention models to produce better captions ~\cite{vinyals2015show,johnson2015densecap}. Furthermore, in ~\cite{johnson2015densecap} a dense captioning method has been proposed, where for a given image, multiple captions are produced and each caption comes with a bounding box. Visual Question Answering (VQA)\cite{Antol2015,Ren2015, malinowski2014multi,Ren2015, agrawal2015vqa,xiong2016dynamic, zhang2015yin} is also related to our problem. It has a deep root in textual question answering ~\cite{bordes2015large,kumar2015ask,weston2014memory}. The goal of textual question answering is to answer a question based on a collection of sentences. 

The major difference between VQA with the VC problem is the existence of a question other than the image or video. This makes the problem harder since the question could be about details of the image or video; however, for the VC problem, any fact about the image can be a correct caption. Some methods use a combination of the question with the image/video through LSTMs ~\cite{malinowski2015ask} and use the output to answer the question. Other methods combine the image features with the words one by one, for instance, the method in ~\cite{xiong2016dynamic} is an extension of ~\cite{kumar2015ask}, and both visual and textural information is input into the dynamic memory networks and converted to a sequence through an RNN with an iterative attention process. In ~\cite{zhang2015yin}, a binary question answering (yes/no) on abstract (unreal) scenes is discussed. Another binary answering problem which verifies existence of a relation between two concepts (for example: dogs eat ice cream) is proposed in ~\cite{sadeghi2015viske} and it uses CNNs to verify the questions. In ~\cite{MovieQA}, it shows another form of VQA, however the questions in this case come as a video and a subtitle. In ~\cite{weston2014memory}, it uses multiple choice questions, but it was demonstrated that the visual information does not contribute much to the final results.

It is clear that the Video-Fill-in-the-Blank (VFIB) problem is very different from the Visual Captioning (VC) problem, since the inputs to these problems are totally different. And the major difference between VFIB problem and the VQA problem is that, the VFIB problem does not have a complete sentence as the ``question"", and the sentence comes as fragments with a blank that can be at anywhere in the sentence. Therefore, we propose a new method to encode the incomplete sentence, and we employ spatiotemporal attention models to capture the object-centric and motion-centric visual features to fill in the blank.

